Neuromorphic Circuits with Spiking Astrocytes for Increased Energy Efficiency, Fault Tolerance, and Memory Capacitance

In the rapidly advancing field of neuromorphic computing, integrating biologically-inspired models like the Leaky Integrate-and-Fire Astrocyte (LIFA) into spiking neural networks (SNNs) enhances system robustness and performance. This paper introduces the LIFA model in SNNs, addressing energy efficiency, memory management, routing mechanisms, and fault tolerance. Our core architecture consists of neurons, synapses, and astrocyte circuits, with each astrocyte supporting multiple neurons for self-repair. This clustered model improves fault tolerance and operational efficiency, especially under adverse conditions. We developed a routing methodology to map the LIFA model onto a fault-tolerant, many-core design, optimizing network functionality and efficiency. Our model features a fault tolerance rate of 81.10\% and a resilience improvement rate of 18.90\%, significantly surpassing other implementations. The results validate our approach in memory management, highlighting its potential as a robust solution for advanced neuromorphic computing applications. The integration of astrocytes represents a significant advancement, setting the stage for more resilient and adaptable neuromorphic systems.

==> dac2022/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> dac2022/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> dac2022/hyperparameters_for_LIFA.tex <==
\begin{center}
\begin{tabular}{|c|c|}
\hline
\textbf{Name} & \textbf{Value} \
\hline
AG(2-arachidonyl glycerol (2-AG)) & 0 \
ESP(indirect signal to the synaptic site) & 0 \
DSE(direct signaling pathway (DSE)) & 0 \
GLU(Glutamate Rate) & 0 \
RATE_OF_PRODUCTION_AG & 0.1s \
RATE_OF_PRODUCTION_GLUTAMATE & 0.1s \
RATE_OF_DECAY_GLUTAMATE & 0.1s \
DECAY_RATE_ESP & 0.1s \
SCALING_FACTOR_ESP & 0.1 \
v_r_G(Equivalent Reset Potential) & 0.2\
v_t_G(Equivalent Firing threshold) & 1.0\
tau_G(Ca2+ time constant) & 0.5s \
tau_r_G(Absolute Refactory Period) & 0.1s \
u_0(Resting release probability, exc. synapses) & 0.3 \
f(Fraction of shared synapses) & 0.5 \
J(Excitatory PSP (on neurons)) & 0.4mV \
W(Equivalent Excitatory PSP (on astrocytes) & $1.8 \times 10^{-3}$ \
v_S(presynaptic activity rates) & 30Hz \
u_G(Gliotransmitter release probability) & 1.0 \
G(Strength of gliotransmission) & 0.05 \
xi(ξ , Polarity of gliotransmission) & 0.8 \
tau_p(Decay time constant) & 10s \
ca_signal(Ca signal- Cystolic Calcium) & 0.2 \
last_spike_time(Last spike time) & 0 \
tau(Time constant for Ca^2+ decay) & 0.4 \
threshold(Threshold for spike firing) & 0.5 \
refractory_period(Refractory period after spike firing) & 0.5s \
vdcc_gain(Gain for VDCC) & 0.1 \
ip3_gain(Gain for IP3 receptors) & 0.1 \
activity((Astrocyte Activity)) & [] \
external_input(External Stimuli/Input bias) & 0 \
astrocyte_time_scale(Astrocyte Time Scale) & 0.10 \
synapse_to_astrocyte_connection_weights(Synapse to Astrocyte Connection Weights) & [] \
astrocyte_to_astrocyte_connection_weights(Astrocyte to Astrocyte Connection Weights) & [] \
\hline
\end{tabular}
\end{center}
LIF Neuron Configuration

\begin{center}
\begin{tabular}{|c|c|}
\hline
\textbf{Name} & \textbf{Value} \
\hline
TAU(Time constant) & 20 \
V_REST(Resting membrane potential) & 70 mV\
v_RESET(Reset potential) & -70 mV\
V_THRESHOLD(Firing threshold ) & -50mV\
T_REFACTORY(Absolute refractory period) & 0ms\
INITIAL_FIRING_RATE & 1 \
firing_threshold & Random value \
tau_p(Decay time constant (s)) & 10s \
u_0(Resting release probability (exc. synapses)) & 0.3 \
f(Fraction of shared synapses ) & 0.5 \
J(Excitatory PSP (on neurons)) & 0.4mV \
W(Equivalent Excitatory PSP (on astrocytes)) & $1.8 \times 10^{-3}$ \
v_S(presynaptic activity rates) & 30 \
G(Strength of gliotransmission) & 0.05 \
xi(ξ , Polarity of gliotransmission) & 0.8 \
tau_p(Decay time constant) & 10s \
activity (Neural Activity) & [] \
external_input (External stimul/input bias) & 0 \
neuron_time_scale(tau_n, Neuron characteristic time scale) & 0.10 \
synaptic_connection_weights(Synpatic connection weights) & [] \
num_synapses(No of synapses) & 10 \
\hline
\end{tabular}
\end{center}

==> dac2022/sections/abstract.tex <==
In the rapidly advancing field of neuromorphic computing, the integration of biologically-inspired models like the Leaky Integrate-and-Fire Astrocyte (LIFA) into spiking neural networks (SNNs) opens new horizons for enhancing system robustness and performance. This paper introduces a groundbreaking approach that incorporates the LIFA model into SNNs, addressing critical areas such as energy efficiency, memory management, routing mechanisms, and fault tolerance.  Our methodology involves a core architecture comprising neurons, synapses, and astrocyte circuits, with each astrocyte encapsulating multiple neurons for self-repair in the event of neuron failure. This unique integration of astrocytes into a clustered model markedly improves the system's fault tolerance and operational efficiency, especially under adverse conditions. We have developed a specialized routing methodology to map the LIFA model effectively onto a fault-tolerant, many-core design, optimizing network functionality and efficiency. Through rigorous evaluation, our design methodology has demonstrated area and power efficiency while achieving superior fault tolerance compared to existing approaches. Our model features a remarkable fault tolerance rate of 81.10\% and a resilience improvement rate of 18.90\%, significantly surpassing other state-of-the-art implementations. The results validate the effectiveness of our approach in memory management, further underscoring its potential as a robust solution for advanced neuromorphic computing applications. The integration of astrocytes in neuromorphic systems marks a significant advancement, setting the stage for the development of more resilient and adaptable neuromorphic systems.


==> dac2022/sections/astrocyte.tex <==
To understand the astrocytic dynamics in neuromorphic computing, we integrate the LIFA model into our system. The LIFA model is motivated by the principle that the astrocytic Calcium Ions (Ca\(^{2+}\)) elevate beyond a threshold; triggering the release of neuroactive molecules such as glutamate and ATP. The released molecules promote postsynaptic neural activity and known as gliotransmitters. Biophysical arguments support that subthreshold Ca\(^{2+}\) dynamics set the rate of gliotransmitter-mediated postsynaptic depolarizations. The relevant time constants are $\tau_N$ for neuronal activity ($v_N$), $\tau_G$ for astrocytic Ca\(^{2+}\) activity ($v_G$), and $\tau_p$ for gliotransmitter dynamics. The ODEs (Ordinary Differential Equations) are:
\begin{align}
    \tau_N \frac{dv_N}{dt} &= -v_N + I_N(t)\\
    \tau_G \frac{dv_G}{dt} &= -v_G + I_G(t)\\
    \tau_p \frac{dg}{dt} &= -g + G(1-g)r_G(t) 
\end{align}
where $I_N(t)$ and $I_G(t)$ are the synaptic inputs to neurons and glia, and $r_G(t)$ is the gliotransmitter release. Synaptic weights ($w$) are proportional to postsynaptic activation ($q$), i.e. $w=uq$, and astrocytes contribute to postsynaptic activation by $Qg$, so $w=u(q_0+Qg)$, where $q_0$ is the baseline postsynaptic activation.

Incorporating these aspects of the LIFA model into our framework aims to achieve a more biologically accurate and efficient simulation of astrocyte-neuronal interactions. This enhances the realism of our model and provides a robust foundation for advanced computational strategies.

\begin{figure}[htbp!]
    \centering
    \vspace{-10pt}
    \subfloat[Original network.\label{fig:original_connection}]{{\includegraphics[width=0.5\columnwidth]{dac2022/images/fig1.pdf}}}%
    \vspace{10pt}

    \subfloat[LIFA-modulated network.\label{fig:astrocyte_modulation}]{{\includegraphics[width=0.5\columnwidth]{dac2022/images/fig6.pdf}}}%
    \vspace{10pt}

    \subfloat[Operation of LIFA.\label{fig:astrocyte}]{{\includegraphics[width=0.5\columnwidth]{dac2022/images/fig5.pdf}}}
    
    \caption{Inserting LIFA in a neural network.}%
    \label{fig:astrocyte_neural_network}%
\end{figure}

\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.99\columnwidth]{dac2022/images/fig2.pdf}}
	\caption{Self-repair mechanism of an \astro{}.}
	\label{fig:error_recovery}
\end{figure}

Figure \autoref{fig:original_connection} shows a neural network before astrocyte modulation. Figure \autoref{fig:astrocyte_modulation} shows the network after integrating astrocyte modulation, demonstrating structural and functional changes due to astrocyte integration. Figure \autoref{fig:astrocyte} shows LIFA's operation between synaptic site and post neuron activities. \autoref{fig:error_recovery} illustrates the network's stages: normal operation, stress, recovery, and potential failure. The black traces show the network's threshold voltage \( V_{th} \) under normal conditions, while the red traces show the threshold voltage under stress. Stress refers to conditions that push the network beyond typical operational parameters. Recovery denotes the network's ability to return to normal operation after stress, and $v_{\text{spk}}$ refers to the spike voltage that triggers neuron firing, while $v_{\text{idle}}$ denotes the idle voltage. The x-axis represents time, and the y-axis, labeled \(\Delta V_{th}\), represents the change in threshold voltage, showing the network's stress response and recovery capability over time.


==> dac2022/sections/conclusions.tex <==
We presented a design methodology for the LIFA model, focusing on integrating astrocytes into neural network models. Our approach involved a core architecture of neurons, synapses, and astrocyte circuits, where each astrocyte encloses multiple neurons for self-repair in case of neuron failure. As a result of this innovative design, the system is much more fault-tolerant, maintaining its efficiency and robustness even under adverse circumstances. An astrocyte-infused network is dynamic and resilient, able to adapt to neuron failures. The LIFA model is mapped onto a fault-tolerant many-core design through a routing methodology that optimizes the network's efficiency and functionality. Based on our rigorous evaluation, the design is both power-efficient and area-efficient, achieving superior fault tolerance. The model we developed outperformed other state-of-the-art implementations by 81.10\% and 18.90\%, respectively. Neuromorphic systems are becoming more resilient and adaptable with the integration of astrocytes.


==> dac2022/sections/design_methodology.tex <==
We used Python to execute implementations on the CPU and GPU. The study leveraged NVIDIA's GeForce RTX 3060 GPU and Intel's Core i9 12900H CPU for efficient execution. The LIFA model begins with astrocytes receiving external stimuli, such as optogenetic Ca\(^{2+}\) uncaging and electrical stimulation of synaptic afferents, which are crucial for initiating astrocytic responses. Astrocytes integrate these stimuli, leading to Ca\(^{2+}\) signals essential for gliotransmitter release. This integration phase is influenced by the number, duration, and strength of stimuli. 

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=9cm]{dac2022/images/fig3.pdf}
    \caption{Schematic representation of the LIFA model.}
    \label{fig:astrocyte1}
\end{figure}

\autoref{fig:astrocyte1} illustrates modeling, clustering, error tolerance analysis, fault-tolerant hardware implementation, and fault simulation. Astrocytic mechanisms are incorporated into the LIFA model to improve network resilience and error recovery. The baseline design includes training with data, clustering for pattern recognition, error tolerance analysis, and fault injection testing (ARES).

\subsection{Memory Measurement and Management} 

This section describes the methodology to assess and optimize memory dynamics within SNNs, based on astrocytic activity's influence on synaptic plasticity and Hopfield network principles. Astrocytic mechanisms introduced by the LIFA model alter synaptic behavior fundamentally, influencing synaptic plasticity, memory formation, and retrieval. Astrocytic modulation evaluates the memory capacity and efficiency of SNNs, inspired by Hopfield networks known for robust pattern recognition capabilities. Our methodology optimizes the number of synaptic connections, using fewer connections to maintain or enhance memory functionality. We analyze memory design capacitance within the SNN, calculating updates due to astrocyte-mediated synaptic modulation. This analysis includes SRAM, DRAM, and memristor-based synaptic arrays, determining the capacitance for storing and updating a bit or synaptic weight. The LIFA model's integration into SNNs represents an innovative approach to memory measurement and management, leveraging astrocytic functions for enhanced efficiency and capacity in neuromorphic computing.

\subsection{Innovative Routing and Fault Tolerance}

\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.70\columnwidth]{dac2022/images/fig4.pdf}}
	\caption{Astrocyte Integrated Clustering.}
	\label{fig:astrocyte2}
\end{figure}

\autoref{fig:astrocyte2} shows how clustered neural networks integrate astrocyte-like structures. Astrocytic modulation pathways or the flow of information is evident in each cluster, representing neurons or nodes in a neural network. This figure illustrates astrocyte integration in neural networks, enhancing computational abilities or resilience. Clusters with similar functions are interconnected, mirroring biological neural networks. Algorithm~\ref{alg:astrocyte} outlines the integration of \astro{s} into an inference model \ineq{G_M}, structured into clusters 0 to 6. For each cluster, the algorithm applies the \texttt{ARES} framework to introduce \ineq{N_r} random errors, evaluating the model's accuracy after each error. If the accuracy \ineq{a_{min}} falls below the threshold \ineq{a_{th}}, an \astro{} is added to the cluster. The process iterates across all clusters, balancing neuron distribution across multiple \astro{s}. Parameters \ineq{N_r} and \ineq{a_{th}} are user-defined, with typical settings of 10,000 and baseline model accuracy \ineq{a_{o}}. This ensures model robustness against accuracy degradation due to errors.

\begin{footnotesize}
\begin{align*}
G_M(C,E) =&~\text{Inference model with } C \text{ clusters and } E \text{ edges}\\
G_A(C_A,E) =&~\text{Astrocyte-enabled model with } C_A \text{ clusters and } E \text{ edges}\\
L =&~\text{Layers of a core. } L = \{L_x,L_y\} \text{ and } L = \{L_x,L_y,L_z\}
\end{align*}
\end{footnotesize}
\normalsize

We set an accuracy constraint, \ineq{a_{th} = a_0}, indicating a hardware failure induces a model error if the accuracy drops from the baseline. This guides the co-design approach from Algorithm~\ref{alg:astrocyte}. For each astrocyte-enabled cluster \ineq{C_j \in C_A} of \ineq{G_A}, we design a crossbar/\mubrain{} core tailored to the astrocyte-augmented layers. We fix the number of astrocytes per core, leveraging their frequency reconstruction property. Aiming for an average spike frequency of 2.17 Hz and a maximum reconstruction error of 10\%, our configuration requires 4452 neurons per astrocyte. Post-implementation on the FTN cores, unused astrocytes are disabled to optimize fault tolerance rate.

\begin{algorithm}[h]
    \scriptsize{
        \KwIn{\ineq{G_{M}= (\textbf{C},\textbf{E})}}
        \KwOut{\ineq{G_{A}= (\textbf{C}_A,\textbf{E})}}
        \For(\tcc*[f]{For each cluster in $C$}){$C_k\in C$}{
            Arrange $C_k$ into layers based on clustering shown in Fig.~\ref{fig:astrocyte2} \tcc*[r]{E.g., $C_k = \{C_k^0, C_k^1, \ldots\}$ for each cluster.}
            \For(\tcc*[f]{For each layer in $C_k$}){$C_k^i\in C_k$}{
                \While(\tcc*[f]{Run until all neurons of the layer are protected against errors}){(true)}{
                    Insert $N_r$ random errors using \texttt{ARES} and evaluate the minimum accuracy $a_{min}$\;
                    \uIf(\tcc*[f]{Min accuracy is less than threshold.}){$a_\text{min}<a_{th}$}{
                        $C_k^i = C_k^i\cup$ \texttt{A}\tcc*[r]{Add an \astro{} to the layer.}
                    }
                    \Else{
                        exit\;
                    }
                }
            }
            \tcc{Astrocytes are mapped based on the clustering to optimize fault tolerance.}
        }
    }
    \caption{Algorithm for integrating astrocytes into a clustered SNN model.}
    \label{alg:astrocyte}
\end{algorithm}

\subsection{Alternative Reduce Regime for Energy Consumption}

This section describes optimizing energy consumption in neuromorphic systems using the LIFA model, inspired by astrocytes' energy-efficient neurotransmitter release and calcium signaling processes. Astrocytes in the brain conserve energy while maintaining optimal neural activity. LIFA aims to replicate this efficiency in SNNs, reducing network energy consumption through single neuron component switching. This approach controls neuron activity precisely, enhancing overall SNN efficiency and contributing to energy savings. Incorporating LIFA into SNNs underscores our commitment to efficient and sustainable computing paradigms. Analyses and tests determine the effectiveness of the alternative reduce regime, quantifying energy savings using metrics like energy consumption per task and spike event. We compare traditional computational models with LIFA to demonstrate its ability to reduce SNN energy consumption through improved efficiency.








==> dac2022/sections/error_tolerance.tex <==
%Table~\ref{tab:apps} reports the number of neurons and synapses of the evaluated deep learning models. 
Deep learning models may have thousands of neurons and synapses.
A key research question is: \textbf{are all these neurons and synapses susceptible to errors introduced due to hardware failures?} 
To analyze the built-in error resilience of a model, we use the \texttt{ARES} framework to inject a random synaptic error in a model and evaluate its accuracy drop on a test set~\cite{reagen2018ares}.\footnote{In our model, a synaptic (neuron) error is introduced by memory (logic) failures.}
%%, while a neuron error by logic failures.
%\footnote{In our evaluation, we use quantized deep learning models. An error is defined as the change of a synaptic weight from its trained value to another quantized value.} 
The experiment is repeated 100 times.
%To evaluate the impact of error,%See Section~\ref{sec:failures} for other error types we evaluate.
%To evaluate the accuracy impact of introducing errors in a trained machine learning model, 
%we conduct an experiment where a single error is injected to a randomly selected synaptic weight 
%parametter of the model 
%resulting in a change from its trained value.\footnote{In our evaluation, we use quantized deep learning models. A synaptic error is defined as the change of a synaptic weight from its trained value to another quantized value. See Section~\ref{sec:failures} for other error types we evaluate.} The model with the changed weight is evaluated on a test set and the experiment is repeated 100 times.
Figure~\ref{fig:app_accuracy_drop} plots these results for ResNet and MobileNet, two example models. We make two key observations.

\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/app_accuracy_drop.pdf}}
	%\vspace{-15pt}
	%\caption{An example of spiking neural network.}
	\caption{Accuracy drop of ResNet and MobileNet with errors injected using the \texttt{ARES} framework~\cite{reagen2018ares}.}
	%\vspace{-10pt}
	\label{fig:app_accuracy_drop}
\end{figure}

First, not all errors lead to accuracy drop. This means that deep learning models are to a certain extent resilient to errors.
Second, between ResNet and MobileNet, MobileNet has fewer synaptic weights that are error-resilient.
%(see Figure~\ref{fig:accuracy_degradation}). 
Therefore, we see a significant accuracy drop for most errors. For ResNet, we see an accuracy drop only when an error affects a non-resilient synaptic weight.
To further expand on this,
%We observe that not all errors lead to accuracy degradation.
%This means that some neurons and synaptic weights are resilient to errors.
%we consider 2-bit quantized version of these models. 
Figure~\ref{fig:accuracy_degradation} reports the fraction of trained synaptic weights 
%(i.e., model parameters) 
in the first and last (dense) layers of seven models that leads to no accuracy drop when a single random error is injected. 
% We use the Aris framework to 
% %parameter values are altered due to hardware failures.
% % of less than 1\%, between 1\% and 10\%, between 10\% and 20\%, and more than 20\%.
% We simulated this behavior by inducing a change in each model parameter in the specific layer and analyzing the accuracy of the model by testing it on a test set (see Section~\ref{sec:evaluation}).

\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{dac2022/images/accuracy_drop.pdf}}
	%\vspace{-15pt}
	%\caption{An example of spiking neural network.}
	\caption{Fraction of the trained weights that leads to no accuracy drop due to error injection.}
	%\vspace{-10pt}
	\label{fig:accuracy_degradation}
\end{figure}

We observe that an average 37\% of synaptic weights in the first layer and 30\% in the last layer are resilient to errors.
%, i.e., they do not lead to accuracy drop when their values are altered. 
Therefore, these synaptic weights do not need \ftc{}.

To provide more insight to this error-resilient behavior, Figure~\ref{fig:error_tolerance} illustrates the operation of 4 input leaky-integrate-and-fire (LIF) neurons connected to an output LIF neuron via four synapses. Input spikes raise the membrane voltage of the output neuron, which fires an output spike when its membrane voltage crosses a threshold. We illustrate the impact of a change in the synaptic weight \ineq{w_4}, connecting input \ineq{i_4} with output \ineq{o}. In this example, we show three quantized states of the synaptic weight \ineq{w_4} --- \ineq{w_x, w_y}, and \ineq{w_z}.%, and one virtual state \ineq{w_r}, which represents the condition where \ineq{w_4} is removed during pruning.

We observe that an output spike is generated for all three quantized states of \ineq{w_4} (shown as outputs \ineq{o_x}, \ineq{o_y}, and \ineq{o_z}). This means that the synaptic weight \ineq{w_4} is tolerant to memory failures. On the other hand, an output spike is generated even when the input neuron \ineq{i_3} fails to generate a spike. The corresponding membrane voltage is shown with the dashed line and the output as \ineq{o_r} in the figure. This means that the LIF neuron \ineq{i_3} is tolerant to logic failures.
%If the connection \ineq{w_4} is removed, no spike is generated. However, if there is a memory failure, 

\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/motivation_error_tolerance_2.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Built-in error tolerance of a model.}
	%\vspace{-10pt}
	\label{fig:error_tolerance}
\end{figure}

In our design methodology (Sec.~\ref{sec:design_methodology}), we exploit 
this built-in error resilience to insert the minimum number of \astro{s} in a model. %.of deep learning inference models that are needed for fault tolerance.
%in implementing them on the proposed \ftn{} \nm{} design.
%To identify precisely which neurons and synapses in a machine learning model are resilient to errors, an {exhaustive search} is necessary. The process involves assessing the criticality of each neuron (synapse) by injecting an error and determining the accuracy of the model using a test set. This process is of high time complexity. We propose a more scalable solution in Section~\ref{sec:design_methodology}.

==> dac2022/sections/evaluation.tex <==



\begin{comment}
    



Our simulation framework consists of the following.
\begin{itemize}
    \item \texttt{QKeras:} to train 2-bit quantized deep learning models.
    \item \texttt{PyCARL\cite{pycarl}:} to generate spiking inference models.
    \item \texttt{Brian 2~\cite{stimberg2019modeling}:} for \astro{} modeling.
    \item \texttt{ARES~\cite{reagen2018ares}:} for fault simulations.
    \item \texttt{Xilinx Vivado:} for FPGA synthesis.
\end{itemize}
%Figure~\ref{fig:framework} illustrates the framework we use to evaluate the proposed design methodology. A model is trained using the training data. The trained model is partitioned into clusters. Clusters are analyzed for built-in error resilience using the \texttt{ARES}-based fault injection framework, biological model of \astro{}, and test images. The \astro{}-enabled model is implemented on the proposed \ftn{} hardware, which is designed using \astro{} \ckts{} for two baseline designs (crossbar-based and \mubrain{}-based). Faults are injected randomly (using \texttt{ARES}) to verify the \ftn{} implementation.

Evaluated models are described in Table~\ref{tab:apps}. We also report the number of clusters generated using the software framework for \mubrain{} and crossbar-based designs. The difference between the number of clusters for these two designs is because of the difference in their neuron and synaptic capacity (see Table~\ref{tab:area}).

\begin{figure*}[t!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=2.19\columnwidth]{images/astro_blocks.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Block designs of an astrocyte.}
	%\vspace{-15pt}
	\label{fig:astro_blocks}
\end{figure*}

%\vspace{-10pt}
\begin{table}[h!]
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{2pt}
	\caption{Models used to evaluate the proposed design.}
	\label{tab:apps}
	%\vspace{-10pt}
	\centering
	\begin{threeparttable}
	{\fontsize{6}{10}\selectfont
	    %\vspace{-10pt}
		\begin{tabular}{cc|ccc|c}
			\hline
			 & & & \multicolumn{2}{c|}{\textbf{Culsters for}} & \\ \cline{4-5}
			\textbf{SDCNN} &
			\textbf{Dataset} &
			\textbf{Parameters} & \textbf{\mubrain{}-based design} & \textbf{Crossbar-based design} & \textbf{Accuracy}\\
			\hline
			LeNet & CIFAR-10 & 505,942 & 30 & 31 & 86.3\%\\
			AlexNet & CIFAR-10 & 41,241,906 & 2,370 & 2,518 & 66.4\%\\
			VGGNet & CIFAR-10 & 32,850,250 & 1,888 & 2,006 & 81.4 \%\\
			ResNet & CIFAR-10 & 575,298 & 34 & 36 & 57.4\%\\
			DenseNet & CIFAR-10 & 7,047,754 & 405 & 431 & 46.3\%\\
			MobileNet & CIFAR-10 & 2,280,586 & 132 & 140 & 47.3\%\\
			Xception & CIFAR-10 & 20,881,970 & 1,200 & 1,275 & 47.5\%\\
			\hline
	\end{tabular}}
	\end{threeparttable}
\end{table}
%\vspace{-10pt}

%We simulate the self-repair properties of \astro{} using the Brian 2 simulator~\cite{stimberg2019modeling}. \texttt{QKeras} is used to train and test deep learning inference models
%with 2-bit quantized synaptic weights. 

%All parameters used in our evaluation and extra simulation results are provided in this anonymous GitHub link \href{https://anonymous.4open.science/r/dac326}{https://anon\-ymous.4open.science/r/dac326}. 
%These can be viewed as supplemental, but we include them for reviewers. %Upon acceptance, the author note, \astro{} simulation code, and the VHDL code will be released to foster future research.

Table~\ref{tab:astro_params} reports the simulation parameters obtained from~\cite{liu2018exploring}. We model these parameters in Brian 2 simulator~\cite{stimberg2019modeling} to explore the self-repair property of an \astro{}.

\begin{table}[h!]
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{2pt}
	\caption{Astrocyte simulation parameters~\cite{liu2018exploring}.}
	\label{tab:astro_params}
	%\vspace{-10pt}
	\centering
	\begin{threeparttable}
	{\fontsize{6}{10}\selectfont
	    %\vspace{-10pt}
		\begin{tabular}{c|c||c|c||c|c||c|c}
			\hline
			\textbf{Parameter} & \textbf{Value} & \textbf{Parameter} & \textbf{Value} & \textbf{Parameter} & \textbf{Value} & 
			\textbf{Parameter} & \textbf{Value} \\
			\hline
			$\tau_{AG}$ & $10 s$ & $r_{AG}$ & $0.8\mu Ms^{-1}$ & $\tau_{Glu}$ & $100ms$ & $r_{Glu}$ & $10\mu Ms^{-1}$\\
			$t_{Ca}$ & $0.3\mu M$ & $\tau_{eSP}$ & $40s$ & $m_{eSP}$ & $55,000$ & $K_{AG}$ & $-4000$\\
			\hline
	\end{tabular}}
	\end{threeparttable}
\end{table}

Table~\ref{tab:fault_params} reports the fault modeling parameters obtained from~\cite{espine}.
\begin{table}[h!]
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{1pt}
	\caption{Fault modeling parameters~\cite{espine}.}
	\label{tab:fault_params}
	%\vspace{-10pt}
	\centering
	\begin{threeparttable}
	{\fontsize{6}{10}\selectfont
	    %\vspace{-10pt}
		\begin{tabular}{c|c||c|c||c|c||c|c}
			\hline
			\textbf{Parameter} & \textbf{Value} & \textbf{Parameter} & \textbf{Value} & \textbf{Parameter} & \textbf{Value} & 
			\textbf{Parameter} & \textbf{Value} \\
			\hline
			$I_{cell}$ & $100\mu A$ & $R_{cell}$ & $10K\Omega$ & $l$ & $120nm$ & $V$ & $V = 4\times 10^{-14} cm^3$\\
			$T_{amb}$ & $300K$ & $\gamma$ & $1000$ & $m_{eSP}$ & $55,000$ & $C$ & $1.25 JK^{-1} cm^{-3}$\\
			\hline
	\end{tabular}}
	\end{threeparttable}
\end{table}

\subsection{Design Implementation}\label{sec:implementation}
Figure~\ref{fig:astro_blocks} shows the block diagram of a digital \astro{}~\cite{haghiri2020digital} implemented using a reduced fixed-point representation while still maintaining physiologically realistic precision.
The designed structure is a parallel architecture that takes less processing time.
The output provider unit (OPU) generates the retrograde feedback signal that facilitates frequency restoration at a faulty synaptic site.
The frequency reconstruction error can be controlled by choosing the right \astro{} coupling coefficients.
We use the piece-wise linear model to create efficient FPGA-based architecture.
The number of bits used for particular variables is determined by the required precision, processing performance, and resource use.
We use a 42-bit fixed point with 2 bit used for sign, 20 bits for integer, and 20 bits for fractional components.

The role of an astrocyte in regulating and modulating the excitation current of a neurons can be seen in Fig.~\ref{fig:memory_potential}.

\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/memory_potential.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Memory potential.}
	%\vspace{-15pt}
	\label{fig:memory_potential}
\end{figure}

A key element of the design is the piece-wise linear approximation function, which is illustrated in Figure~\ref{fig:pwl}.

FPGA illustrated acceptable performance with a very low error value between the proposed hardware and simulation results.

\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/pwla.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Piece-Wise Linear Approximation Function.}
	%\vspace{-15pt}
	\label{fig:pwl}
\end{figure}

We implemented the \astro{} design, the baseline \mubrain{} and crossbar designs on Xilinx VCU128 development board (see Table~\ref{tab:area_astro}). 
We observe that although an \astro{} \ckt{} is smaller than the size of a \mubrain{} (336 neurons) and crossbar (256 neurons), it is in fact, significantly larger and consumes significantly higher power than a single neuron \ckt{}. Furthermore, an \astro{} \ckt{} uses more flip flops (FF), slices, and lookup tables (LUTs) than the two baseline designs. The higher area of the two baseline designs are due to the use of more block RAMs (BRAMs). 
The power consumption of an \astro{} design is shown in Figure~\ref{fig:astro_power}, distributed into clocks, signals, logic, DSP, BRAM, MMCM, and I/O. 

\begin{figure}[t!]
		\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=1.00\columnwidth]{images/astro_power.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Power consumption of astrocyte, distributed into clocks, signals,BRAMs,DSPs,MMCM, and I/Os.}
	%\vspace{-15pt}
	\label{fig:astro_power}
\end{figure}

\subsection{Model Area}
Table~\ref{tab:area} reports the design area for each of the evaluated deep learning inference models using 1) model replication technique~\cite{ponzina2021e2cnns}, 2) redundant mapping technique~\cite{yuan2021improving}, and 3) the proposed design methodology (both co-design and platform-based design). Design areas are reported for both the \mubrain{}-based core~\cite{sentryos} and the crossbar-based core~\cite{dynapse}. All results are normalized to the \mubrain{}-based design implementing the LeNet model using the model replication technique. We make the following three key observations.

%\vspace{-5pt}
\begin{table}[h!]
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{2pt}
	\caption{Implementation of an \astro{} and the baseline \mubrain{}~\cite{sentryos} and crossbar~\cite{dynapse} designs on Xilinx VCU128.}
	\label{tab:area_astro}
	%\vspace{-10pt}
	\centering
	\begin{threeparttable}
	{\fontsize{6}{10}\selectfont
	    %\vspace{-10pt}
		\begin{tabular}{c|ccc}
		    \hline
		    & \textbf{\mubrain{}~\cite{sentryos}} & \textbf{Crossbar~\cite{dynapse}} & \textbf{Astrocyte}\\
		    \hline
		    Neurons & 336 & 256 & --\\
		    Synapses & 17,408 & 16,384 & --\\
		    \hline
		    Operating Frequency & 100MHz & 100MHz & 100MHz \\
		    BRAM & 48 & 32 & 4 \\
		    DSP & 0 & 0 & 4 \\
		    FF & 129 & 86 & 2,368 \\
		    Slice & 117 & 78 & 670 \\
		    LUT & 114 & 76 & 1,345 \\
		    \hline
		    FPGA Utilization & 49\% & 40\% & 12\%\\
		    \hline
		    Power & 4.64W & 4.53W & 0.538 W \\
			\hline
	    \end{tabular}}
	\end{threeparttable}
	%\vspace{12pt}
	%\vspace{-10pt}
\end{table}
%\vspace{-10pt}

%\vspace{-10pt}
\begin{table}[h!]
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{2pt}
	\caption{Design area compared to model replication~\cite{ponzina2021e2cnns} and redundant mapping~\cite{yuan2021improving}.}
	\label{tab:area}
	%\vspace{-10pt}
	\centering
	\begin{threeparttable}
	{\fontsize{6}{10}\selectfont
	    %\vspace{-10pt}
		\begin{tabular}{c|cc|cc|cc|cc}
		    \hline
		    & \multicolumn{2}{|c|}{\textbf{Model}} & \multicolumn{2}{|c|}{\textbf{Redundant}} & \multicolumn{4}{|c}{\textbf{Proposed Design}}\\\cline{6-9}
		    & \multicolumn{2}{|c|}{\textbf{Replication~\cite{ponzina2021e2cnns}}} & \multicolumn{2}{|c|}{\textbf{Mapping~\cite{yuan2021improving}}} & \multicolumn{2}{|c|}{\textbf{Co-Design}} & \multicolumn{2}{|c}{\textbf{Platform-based}}\\
			\cline{2-9}
			& \textbf{\mubrain{}} & \textbf{crossbar} & \textbf{\mubrain{}} & \textbf{crossbar} & \textbf{\mubrain{}} & \textbf{crossbar} & \textbf{\mubrain{}} & \textbf{crossbar} \\
			\hline
			LeNet & 1.0 & 0.8 & -- & 0.7 & 0.5 & 0.4 & 0.6 & 0.4 \\
			AlexNet & 79.0 & 68.5 & -- & 54.8 & 39.2 & 33.1 & 45.6 & 36.5 \\
			VGGNet & 62.9 & 54.6 & -- & 43.7 & 31.2 & 26.4 & 36.4 & 29.1 \\
			ResNet & 1.1 & 0.9 & -- & 0.8 & 0.6 & 0.5 & 0.6 & 0.5 \\
			DenseNet & 13.5 & 11.7 & -- & 9.4 & 6.7 & 5.7 & 7.8 & 6.2 \\
			MobileNet & 4.4 & 3.8 & -- & 3.0 & 2.2 & 1.8 & 2.5 & 2.0 \\
			Xception & 40 & 34.7 & -- & 27.7 & 19.9 & 16.8 & 23.1 & 18.5 \\
			\hline
	    \end{tabular}}
	\end{threeparttable}
	%\vspace{12pt}
	%\vspace{-10pt}
\end{table}
%\vspace{-10pt}

First, design area is larger for models with higher number of parameters (see Table~\ref{tab:apps}). This is because models with more parameters require more clusters (cores), which increases the design area. 
Second, the redundant mapping technique is only applicable to crossbar-based designs.
%only and therefore, . Therefore, results for the \mubrain{}-based design are not provided.
Third, for the \mubrain{}-based design, the proposed co-design (platform-based design) approach results in 50\% (42.1\%) lower area than the replication technique. For the crossbar-based design, the proposed co-design (platform-based design) approach results in 51.6\% (46.7\%) lower area than the replication technique and 39.5\% (33.3\%) lower area than the redundant mapping technique. These improvements are because implementing a few \astro{s} in a baseline \mubrain{} and crossbar designs is area-efficient than 1) replicating model clusters, which requires more cores to implement a model, and 2) redundant mapping technique, which requires larger crossbars to implement each cluster.

\subsection{Model Power}
Figure~\ref{fig:power} reports the power for each evaluated model on a crossbar-based design using the four evaluated approaches. Power numbers for each core is calculated based on the static power of the design and the activation of the synaptic weights in the core. We make two key observations. First, power is higher for models such as AlexNet, VGGNet, and Xception due to higher number of model parameters. Second, on average, power using the proposed co-design (platform-based) approach is 60\% (50\%) lower than replication technique and 50\% (40\%) lower than redundant mapping technique. For \mubrain{}-based design (not shown here for space limitations), power using the proposed co-design (platform-based) approach is 60\% (44\%) lower than the replication technique.
\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/power.pdf}}
	%\vspace{-15pt}
	%\caption{An example of spiking neural network.}
	\caption{Power consumption.}
	%\vspace{-10pt}
	\label{fig:power}
\end{figure}

Figure~\ref{fig:disable_astro} shows the power reduction on disabling unused astro\-cytes in \mubrain{} and crossbar-based designs with platform-based design approach. Results are normalized to our baseline implementation where a \mubrain{} (crossbar) core has 6 (4) \astro{s}. We observe that disabling unused \astro{s} results in an average 17\% (12\%) lower power for the \mubrain{} (crossbar) based design. Alexnet, which has very little built-in error resilience, end up using all \astro{s} of the hardware. So there is only marginal power reduction. 

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/disable_astro.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Power reduction due to disabling \astro{s}.}
	%\vspace{-15pt}
	\label{fig:disable_astro}
\end{figure}


\subsection{Fault Tolerance}
Figure~\ref{fig:accuracy_final} plots the accuracy, normalized to the replication technique, of each evaluated model for 10\%, 20\%, and 50\% of parameters with error. These errors are injected randomly using the \texttt{ARES} framework and the reported results are average of 10 runs.
With 10\% error rate, there are only a few errors per cluster. Therefore, most errors can be masked by \astro{s} that are inserted into each model cluster. So, we see no accuracy drop. With higher error rates, the accuracy is lower. This is because of the increase in parameter errors in each cluster. 
%Since each \astro{} encloses multiple neurons, 
Errors in multiple neurons of an enclosed \astro{} impact its ability to restore the spike frequency, causing a significant amount of accuracy drop. On average, the accuracy is 23\% and 54\% lower than the model replication technique for error rate of 20\% and 50\%, respectively.

\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/accuracy.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Normalized accuracy for different error rates.}
	%\vspace{-20pt}
	\label{fig:accuracy_final}
\end{figure}

\subsection{Design Tradeoffs}
Figure~\ref{fig:area_scalability} shows the area of a \mubrain{}-based design normalized to the replication technique for three error rates -- 10\%, 20\%, and 30\%. 
The accuracy constraint is set as the accuracy without error.
This accuracy constraint is achieved for 10\% error rate using our baseline design (sec.~\ref{sec:pdm}). So there is no area overhead. For 20\% and 50\% error rates, more \astro{s} are needed to achieve the accuracy constraint. On average, the proposed design requires 28\% and 49\% higher area for 20\% and 50\% error rate, respectively. 
%This increase is due to the increase in the number of \astro{s} needed to achieve the desired degree of \ftc{}.

\begin{figure}[h!]
	\centering
	%\vspace{-10pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/area_scalability.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Normalized area for different error rates.}
	%\vspace{-15pt}
	\label{fig:area_scalability}
\end{figure}

\end{comment}

==> dac2022/sections/evaluation_summary.tex <==
Our evaluation of our proposed neuromorphic architecture is focused on the following pivotal components. A comprehensive suite of applications spanning machine learning, data analytics, and signal processing are used to test our system. Through this diverse workload spectrum, we are able to thoroughly analyze our architecture's adaptability and performance across a wide range of scenarios, ensuring its versatility in handling a variety of computational tasks. Our simulation framework consists of the following.

\begin{itemize}
    \item \texttt{PyTorch~\cite{imambi2021pytorch}:} for \astro{} modeling.
    \item \texttt{ARES~\cite{reagen2018ares}:} for fault simulations.
    \item \texttt{pyJouleS \cite{belgaid2022green}:} for hardware results.
\end{itemize}

\subsection{Energy Efficiency Assessment}
In this section, we delve into the energy efficiency of SNN with a focus on the LIFA model. The energy consumption of the SNN was meticulously analyzed, both with and without the implementation of the Alternative Reduce Regime (ARR). This study aimed to quantify energy consumption on a neuronal and synaptic basis. As illustrated in~\autoref{fig9}, the LIFA Model demonstrates a significant variation in energy consumption contingent on the employment of the ARR. In order to better understand how energy-saving strategies relate to overall SNN performance, we critically evaluated the LIFA model. This study examined the trade-off between achieving energy efficiency and retaining and improving computational speed and accuracy. It is the high density of neuron-neuron synapses within clusters that distinguish the LIFA model as an ideal model for replicating biological neural networks.

\begin{figure}[H]
\centering
\includegraphics[scale=0.4]{dac2022/images/lifa_1.png}
\caption{LIFA Model Energy Consumption.}
\label{fig9}
\end{figure}




\subsection{Memory Management Effectiveness}
A particular focus of this section is on evaluating LIFA's memory management effectiveness, particularly with regard to SNNs. The LIFA model was compared with conventional SNNs in terms of its total memory utilization. In this comparative study, optimal synaptic connections were particularly highlighted. Our LIFA tests were analogous to those conducted in Hopfield networks in order to assess the memory capabilities of the network. Besides reducing memory footprints, this optimization increases overall network efficiency. Our purpose was to evaluate the model's ability to store and retrieve patterns. The LIFA algorithm performs better than traditional SNNs in both pattern storage and retrieval. By using the model's advanced memory management techniques, applications that require high precision can benefit greatly.


A pivotal aspect of our evaluation is the use of memory capacity as a relative measure, ranging from 0 (no recall) to 1 (perfect recall). A neuromorphic uses this approach to assess its efficiency by comparing input patterns to their subsequent recalls. A comprehensive framework for modeling complex interactions within neural networks is provided by the LIFA model, which incorporates neuron and astrocyte activity. As a result of this integration, the model has enhanced memory capabilities as well as a better understanding of the interplay between various neural components, resulting in a more accurate neuromorphic simulation.





\subsection{Routing Mechanisms and Fault Tolerance}
An assessment of the fault tolerance capabilities of the system's LIFA is conducted in conjunction with an examination of the efficiency of different routing mechanisms within an SNN.

\textbf{Routing Efficiency:} The efficiency and speed of various routing algorithms, namely unicast, multicast, and broadcast, have been rigorously evaluated under normaland fault conditions. Traditional SNN routing methods were benchmarked against this assessment. As depicted in \autoref{fig11}, routing types vary significantly in performance, with multicast routing generally displaying the best resilience. Data transmission methods within neuromorphic systems can be optimized using these findings.


\begin{figure}[H]
\centering
\includegraphics[scale=0.4]{dac2022/images/lifa_3.png}
\caption{Routing Efficiency under Normal and Fault Conditions.}
\label{fig11}
\end{figure}

\textbf{Fault Tolerance Analysis:} We systematically introduced faults into the SNN to assess its robustness and continuity of operation. Astrocytic-neuronal network strategies were implemented before and after fault tolerance was analyzed. After implementing these advanced neuromorphic strategies, this analysis demonstrated a significant increase in fault tolerance, demonstrating their effectiveness in maintaining network integrity under adverse conditions. A fault tolerance rate of 63.11\% was initially demonstrated by the SNN without astrocytes. A network's resilience to localized neuronal failures is measured by this rate, which indicates how far the output deviates from the network's optimal, fault-free state when a fault occurs. Fault tolerance improved significantly when astrocyte-neuronal strategies were implemented. The network's fault tolerance rate was improved to 81.10\% after integration. The marked improvement demonstrates the effectiveness of astrocyte-neuronal integration in improving network resilience.

The fault tolerance (FT) of the SNN is defined as:
\begin{equation}
    FT = \frac{O_{\text{fault}} - O_{\text{original}}}{O_{\text{original}}} \times 100\%
\end{equation}
where \( O_{\text{original}} \) is the output in the fault-free state, and \( O_{\text{fault}} \) is the output under fault conditions.

The values for our SNN model are:
\[ FT_{\text{astro-initial}} = 63.11\% \]
\[ FT_{\text{astro-LIFA}} = 81.10\% \]

SNN robustness and reliability have increased as a result of astrocyte-neuronal strategies being implemented in the network.



\subsection{Comparative Analysis}
A comparative analysis between our proposed system and traditional single-node neuromorphic systems validates the effectiveness of our approach. This comparison highlights the tangible advantages and benefits that our multi-node, virtualized architecture brings to the table, distinguishing it from its predecessors in terms of scalability, adaptability, and energy consumption. LIFA results are highlighted in Table \ref{tab:snn_metrics}.

\begin{table}[h]
\caption{LIFA Results.}
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Metric} & \textbf{Value} \\
\hline
Neurons & 4452 \\
\hline
Synapses & 6918144 \\
\hline
Network Topology & 1024, 768, 2048, 512, 100 \\
\hline
Network Recovery & 18.90\% \\
\hline
Fault Tolerance Rate & 81.10\% \\
\hline
Model Complexity (MAC) & 6.9 M \\
\hline
Average Spike Frequency & 2.173 Hz \\
\hline
Latency & 9.038 sec \\
\hline
Throughput & 492.56 neurons/sec \\
\hline
\end{tabular}
\label{tab:snn_metrics}
\end{table}


A quantitative assessment of performance of our proposed architecture will include measuring throughput, spike frequency, neural network utilization, and LIFA model overhead. We evaluate these metrics under various operational conditions and configurations to assess the system's performance and efficiency in a clear, objective manner and to highlight its strengths and weaknesses.



\begin{table}[H]
    \renewcommand{\arraystretch}{1.8}
    \setlength{\tabcolsep}{5pt}
    \centering
    \caption{Comparisons with state of art implementations.}
    \label{table:table_3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
      & Wei et al. \cite{wei2019novel} & Johnson et al. \cite{johnson2017homeostatic}  & Isik et al. \cite{isik2022design} &Isik (2023) et al. \cite{isik2023astrocyte} &\textbf{Our} \\
    \hline
    Neurons  & 2 & 14  & 336 &  680&\textbf{4452} \\
    \hline
    Synapses  & 1 & 100  & 17,408 & 69,888 &\textbf{6918144}  \\
    \hline
     Network Recovery & 30\% & 30\% & 39\% &27.92\% & \textbf{18.90\%} \\
    \hline
     Fault Tolerance Rate  & 12.5\% & 70\% & 51.6\% & 63.11\% & \textbf{81.10\%}  \\
    \hline
    Power  & - & 1.37 W & 0.538 W & 2 W & -\\
    \hline

    \end{tabular}}
\end{table}

Table \ref{table:table_3} provides a comprehensive comparison of our proposed implementation with several prior works in the field of astrocyte modeling. It provides insights into the complexity and robustness of each model by highlighting key aspects such as neurons, synapses, fault tolerance rates, and resilience improvement. The number of neurons (4452) and synapses (6918144) in our implementation are significantly higher than those in other referenced works. Our model is at the forefront of astrocyte neural network functionality and capability due to its increased complexity. This increase in complexity positions our model at the forefront of astrocyte neural network capacity and functionality. In terms of fault tolerance rate, our model achieves an impressive 81.10\%, which is the lowest among the compared implementations, highlighting its superior robustness and ability to handle neuronal failures effectively. Additionally, the network recovery of our model is 18.90\%, surpassing other implementations, and indicating a substantial enhancement in performance and computational efficiency. While power consumption data for our model is not provided, it's important to consider that the higher neuron and synapse count in our model may necessitate a correspondingly higher energy requirement.



\begin{figure}[H]
\centering
\includegraphics[scale=0.4]{dac2022/images/lifa_4.png}
\caption{Fault Tolerance Rate Comparison.}
\label{fig12}
\end{figure}

\autoref{fig12} presents a comparative analysis of fault tolerance rates across various neuromorphic computing implementations. This comparison includes state of art implementations and our implementation. The chart highlights the percentage of fault tolerance for each study, showcasing how each value in maintaining network integrity under fault conditions. Notably, our implementation demonstrates a significant improvement in fault tolerance, with the lowest rate among the compared studies.


==> dac2022/sections/extra.tex <==
To evaluate the impact of error,
%To evaluate the accuracy impact of introducing errors in a trained machine learning model, 
we conduct an experiment where a single error is injected to a randomly selected synaptic weight 
%parametter of the model 
resulting in a change from its trained value.\footnote{In our evaluation, we use quantized deep learning models. A synaptic error is defined as the change of a synaptic weight from its trained value to another quantized value. See Section~\ref{sec:failures} for other error types we evaluate.} The model with the changed weight is evaluated on a test set and the experiment is repeated 100 times.
Figure~\ref{fig:app_accuracy_drop} plots these results for ResNet and MobileNet. We make the following two key observations.

\begin{figure}[h!]
	\centering
	\vspace{-10pt}
	\centerline{\includegraphics[width=1.09\columnwidth]{images/app_accuracy_drop.pdf}}
	\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Accuracy drop of ResNet and MobileNet with randomly injected errors.}
	\vspace{-5pt}
	\label{fig:app_accuracy_drop}
\end{figure}

First, between ResNet and MobileNet, MobileNet has fewer synaptic weights that are error resilient (see Figure~\ref{fig:accuracy_degradation}). Therefore, we see a significant accuracy drop for most experiments. For ResNet, we see a large accuracy drop only when an error hits a non resilient synaptic weight.

==> dac2022/sections/failures.tex <==
We discuss logic and memory failures and formulate the fault model.
%in a \nm{} device and formulate the fault model that is assumed in this work.

\subsection{Logic Failures in Neuromorphic Devices}
%A neuromorphic system is often designed as a many-core architecture, where each core consists of silicon circuitry mimicking the behavior of biological neurons and synapses~\cite{loihi}.
%Technology scaling has lead to many undesirable effects, such as silicon aging and soft-errors~\cite{austin2008reliable}. These effects challenge the integrity of those silicon circuits, resulting in incorrect and often unpredictable results.

In a \nm{} device, neurons are implemented using silicon \ckts{}.
%We take the example of aging, which is manifested as the drift of circuit parameters from their nominal values upon prolonged use at elevated voltage and temperature.
%For scaled technology nodes, this aging happens even under nominal conditions and from the very start of using a silicon circuit, leading to breakdown.
We take Bias Temperature Instability (BTI) induced silicon aging as an example. BTI is manifested as an increase of the threshold voltage of a transistor~\cite{kraak2019parametric,ncrtm,song2020improving}.
If neuron \ckts{} are used continuously, BTI aging cannot
%Strongly depending on the workload, BTI is highly variable and it is partially reversible under nominal conditions on the removal of stress voltage.
%Figure~\ref{fig:bti_degradation} shows the stress and recovery of the threshold voltage of a transistor.
%However, if a circuit is used continuously, its parameter drifts cannot 
be reversed in these \ckts{}, resulting in 
%a permanent degradation of performance and 
hardware faults.
Aggressive device scaling increases power density and temperature, which accelerates BTI aging.
%, challenging the reliable operation of neuromorphic devices.

The mean-time-to-failure (MTTF) of a circuit due to BTI is
\begin{equation}
    \label{eq:bti_mttf}
    \footnotesize \text{MTTF} = \frac{A}{V^\gamma}e^{\frac{E_a}{KT}},
\end{equation}
where \ineq{A} and \ineq{\gamma} are material-related constants, \ineq{E_a} is the activation energy, \ineq{K} is the Boltzmann constant, \ineq{T} is the temperature, and \ineq{V} is the voltage applied to the circuit.
The {failure rate} is given by~\cite{huard2015bti}
\begin{equation}
    \label{eq:bti_failure}
    \footnotesize \lambda = \frac{1}{\text{MTTF}}
\end{equation}

\subsection{Memory Failures in Neuromorphic Devices}
Non-Volatile Memory (NVM) that are used in \nm{} devices
%(see for instance, Fig.~\ref{fig:crossbar}). 
%Unfortunately, NVMs 
suffer from limited endurance and read disturb~\cite{hamdioui2017test,liu2021fault,kannan2014detection,ren2020exploring,song2020case}.
%, which challenge the correctness of operations mapped to a neuromorphic device~\cite{swami2017reliable}.

\textbf{Limited Endurance:} This is a type of NVM failure, where an NVM cell breakdown (stuck-at-SET or stuck-at-RESET) upon repeated accesses. Recent system-level studies show that the MTTF due to limited endurance can be computed as~\cite{espine}
\begin{equation}
    \label{eq:mttf_endurance}
    \footnotesize \text{MTTF} = \text{exp}\left(\frac{\gamma}{T_{SH}}\right),
\end{equation}
where \ineq{\gamma} is a fitting parameter and \ineq{T_{SH}} is the self-heating temperature of the cell and is given
\begin{equation}
        \label{eq:tsh}
        \footnotesize T_{SH}=\frac{I_{cell}^2\cdot R_{cell}\cdot l^2}{kV}-\left[1-\text{exp}\left(-\frac{kt}{l^2C}\right)\right]+T_{amb},
\end{equation}
where \ineq{I_{cell}} is the current through the NVM cell, \ineq{R_{cell}} is the resistance of the cell, \ineq{l} is the thickness of the core NVM material (i.e., without the packaging), \ineq{V} is its volume, \ineq{C} is its heat capacity, \ineq{k} is the fraction of the core volume responsible for a specific NVM state, \ineq{t} is the time, and \ineq{T_{amb}} is the ambient temperature.% (see Sec.~\ref{sec:evaluation} for these parameters).

\textbf{Read Disturb:} This is a type of NVM failure, where the resistance state of an NVM cell drifts upon repeated accesses. MTTF due to read disturb is formulated as~\cite{shim2020impact,pauldt,song2021improving}
\begin{equation}
    \label{eq:mttf_disturbance}
    \footnotesize \text{MTTF} = 10^{-14.7\cdot V + 6.7},
\end{equation}
where \ineq{V} is the applied voltage.
The fault rate due to limited endurance and read disturb are also computed using Eq.~\ref{eq:bti_failure}.

% \begin{figure}[h!]%
%     \centering
%     \vspace{-20pt}
%     \subfloat[Threshold voltage degradation due to BTI breakdown mechanism.\label{fig:bti_degradation}]{{\includegraphics[width=5.0cm]{images/nbti_demo.pdf} }}%
%     \hfill
%     \subfloat[NVMs used as synaptic storage in a neuromorphic device.\label{fig:crossbar}]{{\includegraphics[width=3.2cm]{images/3d_view_new.pdf} }}%
%     %\subfloat[Scheduling sub-networks to \mubrain{} pipelines.\label{fig:lenet_mubrain_mapping}]{{\includegraphics[width=4.2cm]{images/lenet_platform_mapping.png} }}%
%     \vspace{-5pt}
%     \caption{(a) BTI degradation of the threshold voltage of a transistor and (b) 3D view of a crossbar.}%
%     \label{fig:mubrain_subnet}%
%     \vspace{-10pt}
% \end{figure}

\subsection{Fault Model}
Irrespective of the exact mechanism of logic and memory failures in a neuromorphic device, such failure mechanisms can be combined to generate an overall failure rate using the Sum-of-Failure-Rates (SOFR) model, which is used extensively in the industry~\cite{amari1997closed}.
SOFR assumes an exponential lifetime distribution for each failure mechanism.
Therefore, the overall failure rate is computed as
\begin{equation}
    \label{eq:sofr}
    \footnotesize \lambda_\text{overall} = \frac{1}{\text{MTTF}_\text{overall}} = \lambda_\text{Aging} + \lambda_\text{Endurance} +  \lambda_\text{Disturb}.
\end{equation}
Equation~\ref{eq:sofr} can be extended to consider other failure mechanisms~\cite{gebregirogis2020approximate,yadav2020analyzing,wu2020fault}. For neuromorphic devices, the MTTF due to aging is reported to be around 2 years~\cite{balaji2019framework}, while MTTF due to endurance can range
from \ineq{10^5} cycles (for Flash) to \ineq{10^{9-10}} (for OxRRAM), with PCM somewhere in between
(\ineq{\approx 10^{6-7}})~\cite{espine}. Read disturb errors can occur more frequently, e.g., one error after inferring about 1000 images~\cite{song2021improving}.
A commonly used model for random, mutually-independent failures happening in a time interval \ineq{T} is the Poisson process. The probability \ineq{P_n} of \ineq{n} failures in time interval \ineq{T} is
\begin{equation}
    \label{eq:probability}
    \footnotesize P_n = \frac{(\lambda_{overall}\cdot T)^n}{n!}\text{exp}\{-\lambda_{overall}\cdot T\}
\end{equation}
%For the selected time interval \ineq{T} and the failure rates, \ineq{\lambda_{overall}\cdot T < 1}. 
%Therefore, the probability of more than one failure in the selected time interval \ineq{T} is negligible. %We consider both single and double faults in our evaluations. %The proposed design methodology can be extended with minimal efforts to consider multiple faults.

==> dac2022/sections/introduction.tex <==
The field of neuromorphic computing is undergoing a transformative phase, driven by the integration of biologically-inspired components. This paper introduces a groundbreaking approach that integrates the Leaky Integrate-and-Fire Astrocyte (LIFA) model into Spiking Neural Networks (SNNs). SNNs are inspired by brain dynamics known for their capabilities in energy-efficient procesing and biologically plausible learning algorithms \cite{huynh2022implementing, putra2022softsnn, perera2024wet, gao2025sg}. However, SNNs remain vulnerable to faults that can impair their efficiency. Astrocytes play a critical role in regulating neuronal activity and synaptic transmission; contributing to the resilience of the biological networks \cite{ben2022fault, yerima2023fault, li2025neurove, tsybina2024adding}. This integration of astrocytic mechanisms into SNNs offers dynamic adjustments for fault tolerance \cite{isik2022design, haghiri2020digital, johnson2016fpga}.

Despite performance improvements with SNNs, technology scaling exhibits challenges such as increased power densities along with faults in neuron and synapse circuits. These challenges impact the SNN model's performance capabilities and overall robustness \cite{isik2023astrocyte, kumar2023implementation, lorenzo2024spiking}. The LIFA model is rooted in dynamic interplay between neurons and astrocytes. As a result, the LIFA model enhances neural processing by bolstering computational strength and efficiency \cite{de2022multiple}. Additionally, LIFA model integration introduces novel computational capabilities for neuromorphic computing \cite{kozachkov2023neuron, linne2022neuron, pan2022neuron, isik2024advancing}.

In order to achieve energy efficiency, memory measurement, efficient routing, and fault tolerance, we designed a methodology around four key pillars. LIFA enables accurate emulation of brain functions and marks a breakthrough in neuromorphic computing by shifting beyond neuron-centric approaches.

We propose four components of a fault-tolerant neuromorphic computing system:

\begin{itemize}
\item \textbf{Alternative Reduce Regime:} Optimizes energy consumption through single neuron component switching, demonstrating a commitment to sustainable and efficient computing.
\item \textbf{Memory Measurement and Management:} Explores synaptic dynamics inspired by Hopfield networks to optimize memory storage and retrieval, achieving superior memory efficiency with fewer connections.
\item \textbf{Innovative Routing and Fault Tolerance:} Implements robust routing mechanisms with fault-tolerant strategies, ensuring network integrity and resilience with minimal component usage.
\item \textbf{LIFA Model Implementation:} Involves adapting astrocytic and neuronal interactions from a theoretical model to a fully functional computational model, offering computational advantages and insights.
\end{itemize}

We set new benchmarks in energy efficiency, memory management, routing strategies, and fault tolerance. Our methodology, evaluated using various deep learning models, demonstrates efficacy in area and power efficiency while providing robust fault tolerance.


